Cover time of graphs with bounded genus

The cover time of a finite connected graph is the expected number of steps needed for a simple random walk on the graph to visit all vertices of the graph. It is known that the cover time of any finite connected $n$-vertex graph is at least $(1 + o(1)) n \log n$ and at most $(1 + o(1)) \frac{4}{27} n^3$. By Jonasson and Schramm, the cover time of any bounded-degree finite connected $n$-vertex planar graph is at least $c n(\log n)^2$ and at most $6n^2$, where $c$ is a positive constant depending only on the maximal degree of the graph. In particular, the lower bound is established via the use of circle packing of planar graphs on the Riemann sphere. In this paper, we show that the cover time of any finite $n$-vertex graph $G$ with maximum degree $\Delta$ on the compact Riemann surface $S$ of given genus $g$ is at least $c n(\log n)^2/ \Delta(g + 1)$ and at most $(6 + o(1))n^2$, where $c$ is an absolute constant, if $n$ is sufficiently large and three sufficient conditions for $S$ and a circle packing of $G$ filling $S$.

==> review.tex <==
\section{Riemann surfaces, branched covering and conformal mapping} 

A connected Hausdorff space $S$ is a topological surface 
if there is a collection $\{ (U_i, \varphi_i ) \}$ of open 
subsets $U_i$ and a map $\varphi_i\colon U_i \to \RR^2$ homeomorphic to 
an open set of $\RR^2$ such that $S = \bigcup_i U_i$ and for 
$U_i, U_j$ such that $U_i\cap U_j \neq \emptyset$, 
$\varphi_i\circ \varphi_j^{-1}\colon \varphi_j(U_i\cap U_j) 
\to \varphi_i(U_i\cap U_j)$ is homeomorphic. 
We call $ (U_i, \varphi_i)$, $\{ (U_i, \varphi_i) \}_i$, and 
$\varphi_i\circ \varphi_j^{-1}$ a chart,
an atlas of $S$ and a transformation map, respectively. 
We set the positive orientation of $\RR^2$ by counterclockwise. 
If a topological surface $S = \{ (U_i, \varphi_i) \}$ satisfies that 
$\varphi_i\circ\varphi_j^{-1}$ preserves the positive orientation for any $i,j$, 
$S$ is called orientable. \\ \par 

%\ytnote{what is Riemann surface?}

The Riemann surface $S$ is a $1$-dimensional complex manifold, 
i.e., $S$ is a topological surface whose atlas 
$\{ (U_i, \varphi_i) \}_i$ satisfies that 
$\varphi_i\colon U_i \to \CC$ and 
%of open set $U_i$ and 
% analytic map $\phi_i\colon U_i \to \CC$ such that $\bigcup_i U_i=S$ 
% and 
 for $U_i, U_j$ such that $U_i\cap U_j \neq \emptyset$, 
$\varphi_i\circ \varphi_j^{-1}\colon \varphi_j(U_i\cap U_j) 
\to \varphi_i(U_i\cap U_j)$ is holomorphic. 
By the definition, any Riemann surface is orientable. 
In this paper, we only consider compact (unbordered) Riemann surfaces. 

Let $S_1, S_2$ be two Riemann surfaces.  
We call a map $f\colon S_1 \to S_2$ holomorphic (conformal) if for any $P\in S_1$ and  
any charts $(\varphi_i^1,U_i^1)$ of $S_1$ and 
$\{ (\varphi_j^2,U_j^2)\}$ of $S_2$ such that $P\in U_i^2$ and $f(P)\in U_j^2$, 
 $\varphi^2_j\circ f\circ (\varphi_i^1)^{-1}$ is holomorphic. 
A holomorphic map $f\colon S_1 \to S_2$ is called an isomorphism if $f$ is bijective and $f^{-1}\colon S_2 \to S_1$ is also holomorphic. Then, we say that 
$S_1$ and $S_2$ are isomorphic. 


We define the genus of a compact orientable topological surface $S$ by t
he number of the holes of $S$. 


%\ytnote{intrinsic metric with constant curvature} 
By the uniformization theorem, any Riemann surface $S$ is isomorphic to 
a quotient of a simply connected Riemann surface $\mathbb{X}$, where $\mathbb{X}$
is one of the Riemann sphere $\wh{\CC}$, the complex plane $\CC$, or the open 
unit disk $\mathbb{D}$. 


%\ytnote{analytic map, conformal structure} 
%
%A function $f\colon \CC \to \CC$ is analytic at $a\in \CC$ if 
%there is a positive number $\rho$ such that for any $z\in \CC$ such 
%that $|z-a|<\rho$, $f(z)$ can be represented by a power series 
%\[
% f(z) = \sum_{n=0}^\infty b_n (z-a)^n 
%\] 
%for some $b_n\in \CC$. Then, $f(z)$ is holomorphic at $a$ and 
%$b_n = f^{(n)}(a)/n!$. 



%\ytnote{branch point, branched covering} 

Let $S_1, S_2$ be two Riemann surfaces, and $f\colon S_1 \to S_2$ a nontrivial 
analytic map. 
Then, for any $P \in S_1$ and charts
$z=\varphi_i^1(P) \in \varphi_i^1(U_i^1)$ and $f(P)\in U_j^2$, 
by changing the charts if it is necessary, 
$\varphi_j^2 \circ f\circ (\varphi_i^1)^{-1} (z)$ can be approximated 
as 
\[
 \varphi_j^2 \circ f\circ (\varphi_i^1)^{-1} (z) \sim z^n. 
\] 
%It is known that this $n$ is independent of the choice of 
Then, $n$ is called by the ramification index of $f$ at $P$, denoted 
by $e_P= e_P(f)$. 
We said that $P\in S_1$ is a branch point of $f$ if $e_P >1$. 

We assume that $f$ is nontrivial. Then, it is known that for any 
$Q \in S_2$, the summation 
\[
 \sum_{P \in f^{-1}(Q)} e_P 
\] 
is a constant independent of $Q$. We call this summation the degree 
of $f$. This is denoted by $\deg(f)$. 


%\ytnote{Riemann-Roch, Riemann-Hurwitz} 

Let $S$ be a compact Riemann surface of genus $g$. Then, as a consequence of 
the Riemann-Roch Theorem, we have the following: 
\begin{lem}[{\cite[Corollary~16.12]{forster2012lectures}}]\label{lem:bound-of-degree}
 There is a branched covering $f\colon S \to \wh{\CC}$ whose 
 degree is at most $g+1$. 
\end{lem}
%\nmnote{$\wh{\CC} = \CC \cup \{\infty\}$？}\ytnote{ですね}

%\ytnote{holomorphic covering?} 

On the other hand, let $S_1, S_2$ be compact Riemann surfaces of genus $g_1, g_2$ respectively. 
Then, the following is known: 
\begin{lem}[{Riemann-Hurwitz formula \cite[\S.17.14]{forster2012lectures}}]\label{lem:Riemann-Hurwitz} 
For any analytic map $f\colon S_1 \to S_2$, the following holds: 
\[
 2-2g_1 = \deg(f)(2-2g_2) - \sum_{P\in S_1} (e_P -1). 
\]
\end{lem}

By Lemma~\ref{lem:Riemann-Hurwitz}, an analytic map $f$ appearing in  
Lemma~\ref{lem:bound-of-degree} satisfies 
\begin{align}
 \#\{\text{branch point of } f  \} \leq \sum_{P\in S_1} (e_P -1)  =   2\deg(f) - (2-2g) \leq 4g = O(g). \label{eq:bound-of-num-of-branch-points}
\end{align}


%\ytnote{Conformal, quasi-conformal map} 


Let $\Omega \in \CC$ be a domain, i.e., a connected open subset. 
A function $f$ on $\Omega$ is called ACL (absolutely continuous on lines) 
if for any closed rectangle $R$ in $\Omega$ surrounded by lines parallel to 
the real axis or imaginary axis, $f$ is absolutely continuous 
for almost all lines parallel to real axis or imaginary axis in $R$. 

For an ACL orientation-preserving homeomorphism $f\colon \Omega \to f(\Omega)\subset \CC$, the dilatation of $f$ at $z \in \Omega$ is defined by 
%\[
% D_f(z) = \lim_{\varepsilon\downarrow 0}
% \frac{\max_{w \in C_\varepsilon(z)} |f(w) - f(z)|}
% {\min_{w \in C_\varepsilon(z)} |f(w) - f(z)|}. 
%\] 
\[
 D_f(z) = \frac{|f_z(z)| + |f_{\ol{z}}(z)|}
 { |f_z(z)| - |f_{\ol{z}}(z)|}. 
\] 
For $K \geq 1$, an orientation-preserving homeomorphism 
$f\colon \Omega \to f(\Omega)\subset \CC$ is called $K$-quasiconformal if 
$f$ is ACL on $\Omega$ and $D_f(z)\leq K$ holds for any $z\in \Omega$. 

Let $S_1$ and $S_2$ be two Riemann surfaces. 
An orientation-preserving homeomorphism $f\colon S_1 \to S_2$ is called 
$K$-quasiconformal if for any $p\in S_1$, there is a chart $(\varphi, U)$ 
of $S_1$ (resp. $(\psi, V)$ of $S_2$) such that $p\in U$ (resp. $f(p)\in V$) 
such that $\psi\circ f \circ \varphi^{-1}$ is $K$-quasiconformal. 
%Let $S_1, S_2$ be two Riemann surfaces with given metrics, 
%and $f\colon S_1 \to S_2$ a map between Riemann surfaces. 
%Then, the distortion $D_f(a;\varepsilon)$ of $f$ at $a \in S_1$ with 
%radius $\varepsilon>0$ is defined by 
%\[
% D_f(a;\varepsilon) = 
% \frac{\max_{d_{S_1}(z, a)=\varepsilon}d_{S_2}(f(z), f(a))}
% {\min_{d_{S_1}(z, a)=\varepsilon}d_{S_2}(f(z), f(a))},
%\]
%and the dilatation $D_f(a)$ of $f$ at $a$ is defined by 
%\[
% D_f(a) = \lim_{\varepsilon\downarrow 0} D_f(a; \varepsilon). 
%\]
%Here, $d_{S_i}(z, a)$ is the distance between $z$ and $a$ on $S_i$ with 
%respect to the given metric. 
%We define a quasiconformal map $f\colon S_1\to S_2$ if \ytnote{def of qc map}
%For $K\geq 1$, a quasiconformal map $f$ is $K$-quasiconformal if $f$ satisfies 
%$D_f(a)\leq K$ for any $a\in S_1$. 
We remark that a $K$-quasiconformal map $f$ is conformal if and only if $K=1$. 



%\ytnote{Teichm\"{u}ller space} 

Let $S$ be a compact Riemann surface. For two non-constant analytic 
maps $f_1\colon S \to S_1$, $f_2\colon S \to S_2$ to compact 
Riemann surfaces $S_1, S_2$, $(S_1, f_1)$ and $(S_2, f_2)$ are said 
to be Teichm\"{u}ller equivalent if 
$f_1\circ f_2^{-1}\colon S_2 \to S_1$ is homotopic to a conformal map.  
The set of such equivalence classes is called by the Teichm\"{u}ller 
space for $S$. We set $[S_1]$ as the equivalence class 
including $S_1$. 
On the Teichm\"{u}ller space for $S$, we can define a distance 
between $[S_1]$ and $[S_2]$ by the following manner: 
\[
 d([S_1], [S_2]) = \inf \log K, 
\]
where the inferior is taken for the analytic maps $f_i \colon S \to S_i$ ($i=1,2$) and $K = \inf_{a\in S_1}D_{f_1\circ f_2^{-1}}(a)$. 
In particular, $d([S_1], [S_2])=0$ if and only if $S_1$ is conformally 
equivalent (i.e., isomorphic) to $S_2$. 
%\ytnote{conformally equivalent? mention the reason} 




